The High Inclination Solar Mission

The High Inclination Solar Mission (HISM) is a concept for an out-of-the-ecliptic mission for observing the Sun and the heliosphere. The mission profile is largely based on the Solar Polar Imager concept: initially spiraling in to a 0.48 AU ecliptic orbit, then increasing the orbital inclination at a rate of $\sim 10$ degrees per year, ultimately reaching a heliographic inclination of $>$75 degrees. The orbital profile is achieved using solar sails derived from the technology currently being developed for the Solar Cruiser mission, currently under development. HISM remote sensing instruments comprise an imaging spectropolarimeter (Doppler imager / magnetograph) and a visible light coronagraph. The in-situ instruments include a Faraday cup, an ion composition spectrometer, and magnetometers. Plasma wave measurements are made with electrical antennas and high speed magnetometers. The $7,000\,\mathrm{m}^2$ sail used in the mission assessment is a direct extension of the 4-quadrant $1,666\,\mathrm{m}^2$ Solar Cruiser design and employs the same type of high strength composite boom, deployment mechanism, and membrane technology. The sail system modelled is spun (~1 rpm) to assure required boom characteristics with margin. The spacecraft bus features a fine-pointing 3-axis stabilized instrument platform that allows full science observations as soon as the spacecraft reaches a solar distance of 0.48 AU.

==> SOLA_example_labels.tex <==
This file contains the command names and the labels used in
the associated .tex file.    It is useful to have present file open
as the same time of the .tex file to copy/paste definitions.
When a new definition is added, it is important to keep this file
updated. 

   % Copy/paste of the definitions used in the .tex
\newcommand{\BibTeX}{\textsc{Bib}\TeX}
\newcommand{\etal}{{\it et al.}}

% Definitions for equations
\newcommand{\deriv}[2]{\frac{{\mathrm d} #1}{{\mathrm d} #2}}
\newcommand{\rmd}{ {\ \mathrm d} }
\renewcommand{\vec}[1]{ {\mathbf #1} }
\newcommand{\uvec}[1]{ \hat{\mathbf #1} }
\newcommand{\pder}[2]{ \f{\partial #1}{\partial #2} }
\newcommand{\grad}{ {\bf \nabla } }
\newcommand{\curl}{ {\bf \nabla} \times}
\newcommand{\vol}{ {\mathcal V} }
\newcommand{\bndry}{ {\mathcal S} }
\newcommand{\dv}{~{\mathrm d}^3 x}
\newcommand{\da}{~{\mathrm d}^2 x}
\newcommand{\dl}{~{\mathrm d} l}
\newcommand{\dt}{~{\mathrm d}t}
\newcommand{\intv}{\int_{\vol}^{}}
\newcommand{\inta}{\int_{\bndry}^{}}
\newcommand{\avec}{ \vec A}
\newcommand{\ap}{ \vec A_p}
\newcommand{\bb}{ \vec B}
\newcommand{\jj}{ \vec j}
\newcommand{\rr}{ \vec r}
\newcommand{\xx}{ \vec x}

% Definitions for the journal names
\newcommand{\adv}{    {\it Adv. Space Res.}} 
\newcommand{\annG}{   {\it Ann. Geophys.}} 
\newcommand{\aap}{    {\it Astron. Astrophys.}}
\newcommand{\aaps}{   {\it Astron. Astrophys. Suppl.}}
\newcommand{\aapr}{   {\it Astron. Astrophys. Rev.}}
\newcommand{\ag}{     {\it Ann. Geophys.}}
\newcommand{\aj}{     {\it Astron. J.}} 
\newcommand{\apj}{    {\it Astrophys. J.}}
\newcommand{\apjl}{   {\it Astrophys. J. Lett.}}
\newcommand{\apss}{   {\it Astrophys. Space Sci.}} 
\newcommand{\cjaa}{   {\it Chin. J. Astron. Astrophys.}} 
\newcommand{\gafd}{   {\it Geophys. Astrophys. Fluid Dyn.}}
\newcommand{\grl}{    {\it Geophys. Res. Lett.}}
\newcommand{\ijga}{   {\it Int. J. Geomagn. Aeron.}}
\newcommand{\jastp}{  {\it J. Atmos. Solar-Terr. Phys.}} 
\newcommand{\jgr}{    {\it J. Geophys. Res.}}
\newcommand{\mnras}{  {\it Mon. Not. Roy. Astron. Soc.}}
\newcommand{\nat}{    {\it Nature}}
\newcommand{\pasp}{   {\it Pub. Astron. Soc. Pac.}}
\newcommand{\pasj}{   {\it Pub. Astron. Soc. Japan}}
\newcommand{\pre}{    {\it Phys. Rev. E}}
\newcommand{\solphys}{{\it Solar Phys.}}
\newcommand{\sovast}{ {\it Soviet  Astron.}} 
\newcommand{\ssr}{    {\it Space Sci. Rev.}} 

%%%%%%%%%%%%%%%% Roadmap of the paper with all the labels %%%%%%%%%%%%%%%%%%%%%%%%
%%%% (with the exception of citations since author-year is easy to remember) %%%%%
1 Section~\ref{S-Introduction}
2 Section~\ref{S-general}
  Section~\ref{S-text}
  Section~\ref{S-labels}
3 Section~\ref{S-features}
  Section~\ref{S-equations}
   Section~\ref{S-simple-equations}
     Equation~(\ref{Eq-H-def})
   Section~\ref{S-array-equations}
     Equation~(\ref{Eq-A-B})
     Equation~(\ref{Eq-H-B})
     Equation~(\ref{Eq-H-N})
   Section~\ref{S-long-equations}
     Equation~(\ref{Eq-dH-Phi})  
  Section~\ref{S-figures}
  Section~\ref{S-tables}
  Section~\ref{S-references}
  Section~\ref{S-BibTeX}
  Section~\ref{S-Miscellaneous}
4 Section~\ref{S-Conclusion}

A Appendix~\ref{S-appendix}
 
 1 Figure~\ref{F-simple}
 2 Figure~\ref{F-4panels}
 3 Figure~\ref{F-rotate-cut}
 4 Figure~\ref{F-appendix}

 1 Table~\ref{T-simple}
 2 Table~\ref{T-complex}
 3 Table~\ref{T-appendix}

%%%%%%%%%%%%%%%%%%%% Results for the citation commands %%%%%%%%%%%%%%%%%%%%%%%%  
\cite{Kusano04}          : (Kusano \etal, 2004)
\cite{Kusano04,Berger03} : (Kusano \etal, 2004; Berger, 2003)
\inlinecite{Brown99}     : Brown, Canfield, and Pevtsov (1999)
\opencite{Brown99}       : Brown, Canfield, and Pevtsov, 1999
\citeauthor{Brown99}     : Brown, Canfield, and Pevtsov
\shortcite{Brown99}      : (1999)
\citeyear{Brown99}       : 1999
(\opencite{Berger84}, \citeyear{Berger03}) 
                         : (\opencite{Berger84}, \citeyear{Berger03})



==> inst_spec_table.tex <==


\begin{table}[tbhp]
\centering
\begin{footnotesize}
 \begin{tabular}{|c|c|c|c|c|c|c|c|} 
%   &      &             &              &         &      &       &  \\
 \hline
 Instrument & Doppler    & Coronagraph & Magnetometer & Faraday & Ion & Electrical & Search \\
            & \& Stokes  &             &              & Cup     & Spectrometer & Antennas   & Coil \\
            & Imager     &             &              &         &      &       & Magnetometer \\
 \hline
 \hline
 Science & 1, 2, 5 & 2, 5 & 2, 5 & 2, 3, 5 & 2, 4, 5 & 2, 5 & 2, 5 \\
 Goals\dagger   & & & & & & &\\
 
 \hline
 Orientation & Sun       & Sun         & N/A          & Sun       & Sun & 120 deg    & N/A  \\
             & Pointing  & Pointing    &              & Pointing  & Pointing & apart      & \\
 \hline
 Field of   & $1.5^{\circ}\times 1.5^{\circ}$ & $16^{\circ}$ &
            N/A & $120^{\circ}$ & $60^{\circ}$ & $\sim 2\pi$ & N/A \\
 Regard     &&&&&&& \\
 \hline
 Pointing & $30'$ of & 2' of    &  N/A  & ? & ? & ? & ? \\
 Accuracy & Sun ctr  & Sun ctr  &  N/A  & ? & ? & ? & ? \\
 \hline
 Pointing & $30'$ of & 2' of    &  N/A  & ? & ? & ? & ? \\
 Knowledge & Sun ctr  & Sun ctr  &  N/A  & ? & ? & ? & ? \\
 \hline
 \hline
 Pointing & $20"/10\,\mathrm{s}$ & $7"/\mathrm{s}$ &                 &         &      &       &  \\
 Stability  &      &             &              &         &      &       &  \\
 \hline
 Power & $37\,\mathrm{W}$   & $15\,\mathrm{W}$  &  $2 \times 0.3\,\mathrm{W}$&  $3.5\,\mathrm{W}$& $4.2\,\mathrm{W}$
            & $3 \times 0.3\,\mathrm{W}$     &  $13\,\mathrm{W}$ \\
       &                    &                   &              &         &      &       &  \\
 \hline
 Data    &  75 kbps &  40 kbps &   0.6 kbps  &   0.2 kbps  &  0.2 kbps    &   \multicolumn{2}{|c|}{5 kbps}      \\
 Volume  &      &             &              &         &      &       \multicolumn{2}{|c|}{}  \\
 \hline
 Sensor  & $ 13 \mathrm{kg}$  & $8\,\mathrm{kg}$  &  $2\times 0.15\,\mathrm{kg}$ & $2.1\,\mathrm{kg}$  &  $1.41\,\mathrm{kg}$ 
 &  $3 \times 1.4\,\mathrm{kg}$   &  $1\,\mathrm{kg}$\\
 Mass   &      &             &              &         &      &       &  \\
 \hline
 Electronics \\
 Mass \\
 \hline
 Sensor \\
 Dimensions \\
 \hline
 Mounting \\
 Restrictions \\
 \hline
 \end{tabular}
 \end{footnotesize}
 \label{tbl:inst}
\end{table}
